A Probabilistic Design Method for Fatigue Life of Metallic Component

In the present study, a general probabilistic design framework is developed for cyclic fatigue life prediction of metallic hardware using methods that address uncertainty in experimental data and computational model. The methodology involves (i) fatigue test data conducted on coupons of Ti6Al4V material (ii) continuum damage mechanics based material constitutive models to simulate cyclic fatigue behavior of material (iii) variance-based global sensitivity analysis (iv) Bayesian framework for model calibration and uncertainty quantification and (v) computational life prediction and probabilistic design decision making under uncertainty. The outcomes of computational analyses using the experimental data prove the feasibility of the probabilistic design methods for model calibration in presence of incomplete and noisy data. Moreover, using probabilistic design methods result in assessment of reliability of fatigue life predicted by computational models.

==> Makefile <==
all:	all_texs

clean: clean_texs clean_exec

clean_texs:
	rm -f *.aux
	rm -f *.log
	rm -f *.dvi
	rm -f *.toc
	rm -f *.blg
	rm -f *.idx
	rm -f *.bbl
	rm -f paper_0_main*.ps
	rm -f *.out
	rm -f *.nav
	rm -f *.synctex.gz
	rm -f *.snm

clean_exec:
	rm -f *~

#OBJS_convert = \
#	rawfigs/xyz.eps \
#	rawfigs/abc.eps

# $(OBJS_convert)

all_texs:
	pdflatex paper_fatigue_uq_revised.tex
	pdflatex paper_fatigue_uq_revised.tex
	bibtex   paper_fatigue_uq_revised
	pdflatex paper_fatigue_uq_revised.tex
	pdflatex paper_fatigue_uq_revised.tex


.SUFFIXES: .eps .png .jpg

%.eps: %.png
	convert $< $(basename $<).eps

%.eps: %.jpg
	convert $< $(basename $<).eps

